Geometric feature performance under downsampling for EEG classification tasks

We experimentally investigate a collection of feature engineering pipelines for use with a CNN for classifying eyes-open or eyes-closed from electroencephalogram (EEG) time-series from the Bonn dataset. Using the Takens' embedding--a geometric representation of time-series--we construct simplicial complexes from EEG data. We then compare $\epsilon$-series of Betti-numbers and $\epsilon$-series of graph spectra (a novel construction)--two topological invariants of the latent geometry from these complexes--to raw time series of the EEG to fill in a gap in the literature for benchmarking. These methods, inspired by Topological Data Analysis, are used for feature engineering to capture local geometry of the time-series. Additionally, we test these feature pipelines' robustness to downsampling and data reduction. This paper seeks to establish clearer expectations for both time-series classification via geometric features, and how CNNs for time-series respond to data of degraded resolution.

==> deprecated/acknowledgements_and_impacts.tex <==
% \section*{Acknowlegements}

% We extend heartfelt appreciation to Will Chernoff for excellent feedback on the manuscript including a careful review of the possible implications of this work, leading to the broader impacts section. 

% We also thank Dan Marthaler, Sven Schmit, Janu Verma, and Hector Yee for feedback and comments on the manuscript. 

\section*{Broader Impacts}

As the primary application of study for these experiments lies within the medical space, both positive and negative applications jump to mind. Large, high-resolution datasets both for training and evaluation come at the benefit of those in developed and wealthy communities. Our research --  through its focus on developing methods robust to degradation -- provides an opportunity for an improvement in prediction methods in lower fidelity data regimes; i.e. methods designed with downsampling and data reduction in mind alleviate needs for larger and more complete datasets.

The present study examines EEGs and eye states, which could easily extend to other ailments. More accurate models for predicting seizure, for example, could greatly benefit those privileged enough to share characteristics with those used to train the model in the first place. But what of those not sampled?

As (\cite{Hall-rep}) has observed: Blacks, women, and the elderly have historically been excluded from clinical trial research. Such arrangements can lead to what (\cite{Veinot-intentions}) has referred to as intervention-generated inequalities (IGI), a social arrangement where one group gets better, while others don't. On top of their original ailments, groups left out are burdened with continued medical involvement and the associated costs (e.g. additional tests, transportation, childcare, and missed opportunities).

We offer the following suggestions for those in the medical industry hoping to combat some of this inequity: 1. Insist on multiple representative datasets including those from underrepresented groups -- incentivization where appropriate. 2. Identify and assist in eliminating barriers to involvement in data collection or diagnostics. 

==> deprecated/appendices.tex <==
\section{Downsampling}

\subsection{Time series downsampling}
    % We consider the following division of downsampling methods, faithful and unfaithful. We call a downsampling \textit{faithful} if the downsampled time series is a subsequence of the original time series. Methods which summarize the data, and thus are unfaithful, are popular for a variety of smoothing applications.

    % Additionally, we will think of the distribution of points in the downsample with respect to the original sequence. In the simplest case of downsampling, selecting the first element of evenly spaced buckets, we see that the distribution is extremely uniform. We lightly touch on methods which do not sample uniformly, and in our discussion of dynamic bucketing, tactically break this rule.
    % We refer to \textit{downsample resolution} as the number of points in a time series after downsampling, and it's inverse as the \textit{downsampling rate}.
    
    We consider a downsampling a selection of a subsequence of points, or a smaller set of points that summarize the timeseries. We assume the timeseries has $n+2$ points, and construct a downsample of $m+2$ points.
    
    \textbf{Naive Bucketing}: Select the first and last points of the timeseries; cover the the rest of the points with $m$ even-width intervals(up to integer rounding). We call this a \textit{bucketing}.  
    
    Consider a sequence of sequences:
    \begin{equation*}
        \left\lbrace\left\lbrace x_0 \right\rbrace, \left\lbrace x_1,\ldots,x_k\right\rbrace, \left\lbrace x_{k+1},\ldots,x_{2k}\right\rbrace, \ldots, \left\lbrace x_{(m-1)k+1},\ldots,x_{mk}\right\rbrace, \left\lbrace x_{n+1} \right\rbrace\right\rbrace
    \end{equation*}
    and for simplicity, call the sub-sequences $\left\lbrace{b_i}\right\rbrace_{0\leq i\leq n+1}$ such that $b_0 = \left\lbrace x_0 \right\rbrace$, $b_{n+1} = \left\lbrace x_{n+1} \right\rbrace$, and $b_j = \left\lbrace x_{(j-1)k + 1}\ldots x_{(j-1)k} \right\rbrace$, we refer to these as \emph{buckets}.
    
    \textbf{Dropout:} For each bucket, select the first point in the subsequence.
    
    \textbf{Bucket Averaging:} For each bucket in a naive bucketing, average the $x$ and $y$ coordinates and take this as the reprsentative point; take also the first and last points.

    For a bucket, we compute the 2-dimensional average of the points contained within: $\mu_j$. For convenience of notation, we write elements of $b_i$, as $\left\lbrace x^j_i\right\rbrace$. 
    
    % Finally, we use the notations $\prescript{x}{}{-}$ and $\prescript{y}{}{-}$ to denote the $x$ and $y$ coordinates of points, e.g. $\prescript{x}{}{\mu_j}=\hat{x}$ and $\prescript{y}{}{\mu_j}=\hat{y}$.

    % \textbf{Median-Mode Downsample:} Given the buckets as before, compute the optima of the time series and label the corresponding buckets $b_{max}$, and $b_{min}$. For each other bucket $b_j$ with unique modes of $y$-values, assign the central most point with such $y$-value to the bucket as a representative. Finally, for all remaining buckets, assign to them their median values. 
    
    \textbf{Largest-Triangle Three-Bucket Downsample (LTTB)} We compute the subsequence via the optimization problem:
    \begin{equation*}
        \textbf{compute } l_{i} = \argmax_{x^j_i} \mathbf{\triangle}\left({l_{i-1}, x^j_i, \mu_{i+1}}\right)\text{ such that } l_{0} = b_0 \text{ and } \mu_{n+1} = b_{n+1}.
    \end{equation*}
    The sequence $\left\lbrace l_0,\ldots, l_{n+1}\right\rbrace$ is the \emph{largest triangle three bucket downsample.} For more details and intuition around this construction we recommend the original paper.

    \begin{remark}
        This is computed via a recursive optimization process iterating through the buckets; a non-recursive formulation to find the global optima is also possible. The distinction between these two solutions is that in the recursive solution each optimization is conditioned on the previous bucket, where-as the global solution conditions on all buckets simultaneously.
    \end{remark}
    
\subsection{Dynamic downsampling}

In the above bucketing strategies, points in all regions of the time series are given equal weight in the downsample. Often times, the lagging-variance of a time series is not uniform across the time-domain. One might expect that regions of higher variance might warrant higher resolutions in the downsample, while low variance might require lower resolutions. A simple implementation of this idea, \textit{(inspired by \cite{sveinn})} is demonstrated in Algorithm \ref{alg:dynamic bucketing}(implementation included in Appendix). Downsampling methods are then applied to this bucketing of the timeseries.
    
\begin{algorithm}
  \caption{Variance weighted dynamic bucketing
    \label{alg:dynamic bucketing}}
  \begin{algorithmic}[1]
    \Require{$\mathcal{B}$ a naive bucketing, and $P$ an iteration count}
    \Statex
    \Function{dynamicbuckets}{$B:List[List[Float]$}
      \Let{$[b_j]$}{$\mathcal{B}$} 
    %   \Comment{$\left\lbrace x^j_i\right\rbrace_{1\leq i \leq k}=b_j$: buckets of $\mathcal{B}$}
      \For{$i \gets 1 \textrm{ to } P$}
        \For{$j \gets 1 \textrm{ to } m$}
            \Let{$S(b_j)$}{$SSE(OLS(b_j))$}
        \EndFor
        \Let{$z$}{$\argmax_j(S(b_j))$}
        \Let{$b^l_z$}{$\left\lbrace x^z_1, \ldots, x^z_{\floor{k/2}}\right\rbrace$}
        \Let{$b^r_z$}{$\left\lbrace x^z_{\floor{k/2}+1}, \ldots, x^z_k\right\rbrace$}
        \Let{$\mathcal{B}$}{$\mathcal{B}\setminus \left\lbrace b_z\right\rbrace \cup \left\lbrace b^l_z, b^r_z \right\rbrace$}
      \EndFor
      \For{$i \gets 1 \textrm{ to } P$}
        \For{$j \gets 1 \textrm{ to } m+P$}
            \Let{$S(b_j)$}{$SSE(OLS(b_j))$}
        \EndFor
        \Let{$a$}{$\argmin_a(S(b_a)+S(b_{a+1}))$}
        \Let{$b^*_a$}{$\left\lbrace x^a_1, \ldots, x^a_{k}\right\rbrace \cup \left\lbrace x^{a+1}_{1}, \ldots, x^{a+1}_k\right\rbrace$}
        \Let{$\mathcal{B}$}{$\mathcal{B}\setminus \left\lbrace b_a, b_{a+1} \right\rbrace \cup \left\lbrace b^*_a \right\rbrace$}
      \EndFor
      \State \Return{$\mathcal{B}$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

\begin{remark}
    Rather than serially splitting, and then combining buckets to arrive at the rebucketing, it's natural to ask how alternating these operations effects the result. The authors carried out several simulations of this technique and found that convergence to `stable' bucketing took place much more quickly, but produced far worse results with respect to total SSE.
\end{remark}

\subsection{Dynamic downsampling results}

\begin{figure}[ht]
\includegraphics[width=0.9\textwidth]{paper_materials/figures/eeg_eye_results_dynamic_v2.png}
\caption{Experiment results for dynamic bucketing downsampling methods.}
\label{fig:perf_dynamic}
\end{figure}

\section{another}

==> deprecated/conclusions.tex <==
\section{Outcomes}
		We've explored a collection of `experiments' in training and testing CNNs built on EEG data to predict if a patient's eyes are open or closed. The aforementioned experiments primarily sought to establish performance comparisons while varying the feature engineering choice, the chunk size, and the downsampling resolution used.
		
% 		\begin{itemize}
% 		    \itemsep-0.1em 
% 			\item The featurization of the time series; raw values, persistent Betti numbers, or persistent eigenvalues of the Laplacian
% 			\item The amount of data in each sample; chunksize
% 			\item The resolution of the data under downsampling and the type of downsampling used
% 		\end{itemize}

		We established a baseline performance using a raw time series feature set and reproduced performance in (\cite{Umeda2017}) to compare to this baseline. We saw that the performance of this baseline actually outperforms the TDA feature engineered experiment as reported. This suggests that for a task of this type the TDA approach is not SOTA, but may hold value in other regimes, or under more specific hyperparameter tuning. Building on these results, we explored the novel geometric feature engineering method of persistent eigenvalues of the Laplacian. This method also outperforms TDA, but does not significantly outperform the raw time series experiment.

		We showed the performance of these networks under the strain of reduced data samples, and in resolution reduction. The impact on performance as we iterate through the parameter space is relatively smaller for the eigenvalue features, but perform worse than the raw time-series when a significant difference is detectable.

		Finally, we provided a testbed for further iteration on these sorts of prediction tasks, and opened up a discussion around sensor resolution, sample data size, downsampling, feature engineering, and CNNs. The comparison pipelines are easily extensible for further experimentation with this dataset or others. All of the code for feature engineering and testing is available on GitHub.
	
% 	\subsection{Thoughts and future research topics}
    	Variable resolution training has been employed on ImageNet (\cite{DAWNBench}) to dramatically reduce training time, it's interesting to consider the implications of explicitly controlling downsampling schemes for this ansatz. Larger scope, we have left open the question of ``multi-resolution'' sensor networks and the impact on geometric feature engineering and downsampling.
    
    % 	A different approach to these problems is that of $n$-step out predictions, i.e. given a positive label, is it able to be classified $n$ time-steps before it is seen? Additionally, we are interested in extending this work to a larger dataset and multi-node EEG arrays. Finally, see value in filling out the design matrix sketched above for a deeper analysis of learning rates, biases, and other downsampling techniques.

==> deprecated/downsampling.tex <==
\section{Time series downsampling}
    % We consider the following division of downsampling methods, faithful and unfaithful. We call a downsampling \textit{faithful} if the downsampled time series is a subsequence of the original time series. Methods which summarize the data, and thus are unfaithful, are popular for a variety of smoothing applications.

    % Additionally, we will think of the distribution of points in the downsample with respect to the original sequence. In the simplest case of downsampling, selecting the first element of evenly spaced buckets, we see that the distribution is extremely uniform. We lightly touch on methods which do not sample uniformly, and in our discussion of dynamic bucketing, tactically break this rule.
    % We refer to \textit{downsample resolution} as the number of points in a time series after downsampling, and it's inverse as the \textit{downsampling rate}.
    
    We consider a downsampling a selection of a subsequence of points, or a fewer set of points that summarize the timeseries. We assume the timeseries has $n+2$ points, and construct a downsample of $m+2$ points.
    
    \textbf{Naive Bucketing}: Select the first and last points of the timeseries; cover the the rest of the points with $m$ even-width intervals(up to integer rounding). We call this a \textit{bucketing}.  
    
    Consider a sequence of sequences:
    \begin{equation*}
        \left\lbrace\left\lbrace x_0 \right\rbrace, \left\lbrace x_1,\ldots,x_k\right\rbrace, \left\lbrace x_{k+1},\ldots,x_{2k}\right\rbrace, \ldots, \left\lbrace x_{(m-1)k+1},\ldots,x_{mk}\right\rbrace, \left\lbrace x_{n+1} \right\rbrace\right\rbrace
    \end{equation*}
    and for simplicity, call the sub-sequences $\left\lbrace{b_i}\right\rbrace_{0\leq i\leq n+1}$ such that $b_0 = \left\lbrace x_0 \right\rbrace$, $b_{n+1} = \left\lbrace x_{n+1} \right\rbrace$, and $b_j = \left\lbrace x_{(j-1)k + 1}\ldots x_{(j-1)k} \right\rbrace$, we refer to these as \emph{buckets}.
    
    \textbf{Dropout:} For each bucket, select the first point in the subsequence.
    
    \textbf{Bucket Averaging:} For each bucket in a naive bucketing, average the $x$ and $y$ coordinates and take this as the reprsentative point; take also the first and last points.

    For a bucket, we compute the 2-dimensional average of the points contained within: $\mu_j$. For convenience of notation, we write elements of $b_i$, as $\left\lbrace x^j_i\right\rbrace$. 
    
    % Finally, we use the notations $\prescript{x}{}{-}$ and $\prescript{y}{}{-}$ to denote the $x$ and $y$ coordinates of points, e.g. $\prescript{x}{}{\mu_j}=\hat{x}$ and $\prescript{y}{}{\mu_j}=\hat{y}$.

    % \textbf{Median-Mode Downsample:} Given the buckets as before, compute the optima of the time series and label the corresponding buckets $b_{max}$, and $b_{min}$. For each other bucket $b_j$ with unique modes of $y$-values, assign the central most point with such $y$-value to the bucket as a representative. Finally, for all remaining buckets, assign to them their median values. 
    
    \textbf{Largest-Triangle Three-Bucket Downsample (LTTB)} We compute the subsequence via the optimization problem:
    \begin{equation*}
        \textbf{compute } l_{i} = \argmax_{x^j_i} \mathbf{\triangle}\left({l_{i-1}, x^j_i, \mu_{i+1}}\right)\text{ such that } l_{0} = b_0 \text{ and } \mu_{n+1} = b_{n+1}.
    \end{equation*}
    The sequence $\left\lbrace l_0,\ldots, l_{n+1}\right\rbrace$ is the \emph{largest triangle three bucket downsample.} For more details and intuition around this construction we recommend the original paper.

    \begin{remark}
        This is computed via a recursive optimization process iterating through the buckets; a non-recursive formulation to find the global optima is also possible. The distinction between these two solutions is that in the recursive solution each optimization is conditioned on the previous bucket, where-as the global solution conditions on all buckets simultaneously.
    \end{remark}

% \subsubsection{Topological downsampling}

%     Given an \emph{n-step time-delay embeddings} of $\prescript{y}{}{x^j_i}$'s for those points in $b_j$, 

\subsection{Dynamic Bucketing}


    In the above bucketing strategies, points in all regions of the time series are given equal weight in the downsample. Often times, the lagging-variance of a time series is not uniform across the time-domain. One might expect that regions of higher variance might warrant higher resolutions in the downsample, while low variance might require lower resolutions. A simple implementation of this idea, \textit{(inspired by \cite{sveinn})} is demonstrated in Algorithm \ref{alg:dynamic bucketing}(implementation included in Appendix). Downsampling methods are then applied to this bucketing of the timeseries.
    
%     \begin{algorithm}
%   \caption{Variance weighted dynamic bucketing
%     \label{alg:dynamic bucketing}}
%   \begin{algorithmic}[1]
%     \Require{$\mathcal{B}$ a naive bucketing, and $P$ an iteration count}
%     \Statex
%     \Function{dynamicbuckets}{$B:List[List[Float]$}
%       \Let{$[b_j]$}{$\mathcal{B}$} 
%     %   \Comment{$\left\lbrace x^j_i\right\rbrace_{1\leq i \leq k}=b_j$: buckets of $\mathcal{B}$}
%       \For{$i \gets 1 \textrm{ to } P$}
%         \For{$j \gets 1 \textrm{ to } m$}
%             \Let{$S(b_j)$}{$SSE(OLS(b_j))$}
%         \EndFor
%         \Let{$z$}{$\argmax_j(S(b_j))$}
%         \Let{$b^l_z$}{$\left\lbrace x^z_1, \ldots, x^z_{\floor{k/2}}\right\rbrace$}
%         \Let{$b^r_z$}{$\left\lbrace x^z_{\floor{k/2}+1}, \ldots, x^z_k\right\rbrace$}
%         \Let{$\mathcal{B}$}{$\mathcal{B}\setminus \left\lbrace b_z\right\rbrace \cup \left\lbrace b^l_z, b^r_z \right\rbrace$}
%       \EndFor
%       \For{$i \gets 1 \textrm{ to } P$}
%         \For{$j \gets 1 \textrm{ to } m+P$}
%             \Let{$S(b_j)$}{$SSE(OLS(b_j))$}
%         \EndFor
%         \Let{$a$}{$\argmin_a(S(b_a)+S(b_{a+1}))$}
%         \Let{$b^*_a$}{$\left\lbrace x^a_1, \ldots, x^a_{k}\right\rbrace \cup \left\lbrace x^{a+1}_{1}, \ldots, x^{a+1}_k\right\rbrace$}
%         \Let{$\mathcal{B}$}{$\mathcal{B}\setminus \left\lbrace b_a, b_{a+1} \right\rbrace \cup \left\lbrace b^*_a \right\rbrace$}
%       \EndFor
%       \State \Return{$\mathcal{B}$}
%     \EndFunction
%   \end{algorithmic}
% \end{algorithm}
    
    % \begin{enumerate}
    %     \item Consider again, the buckets of points ${b_j}$ as before, but call this sequence $\mathcal{B}_0$ \begin{itemize}
    %         \item Given points $\left\lbrace x^j_i\right\rbrace_{1\leq i \leq k}$ contained in the bucket $b_j$, compute the linear regression minimizing the sum of squares of the residuals to the model. Record this `loss' as $S(b_j)$.
    %         \item For $z=\argmax_j(S(b_j))$, denote $b^l_z=\left\lbrace x^z_1, \ldots, x^z_{\floor{k/2}}\right\rbrace$, and $b^r_z=\left\lbrace x^z_{\floor{k/2}+1}, \ldots, x^z_k\right\rbrace$
    %         \item Define $\mathcal{B}_p$ inductively as the sequence $\mathcal{B}_{p-1}\setminus \left\lbrace b_z\right\rbrace \cup \left\lbrace b^l_z, b^r_z \right\rbrace$
    %     \end{itemize}
    %     \item Assume now buckets $b_j$ from $\mathcal{B}_p$ but we purposely do not take care to notate different values of $k$ depending on $j$. \begin{itemize}
    %         \item Given points $\left\lbrace x^j_i\right\rbrace_{1\leq i \leq k}$ contained in the bucket $b_j$, compute the linear regression minimizing the sum of squares of the residuals to the model. Record this `loss' as $S(b_j)$.
    %         \item For $a=\argmin_a(S(b_a)+S(b_{a+1}))$, denote $b^*_a = \left\lbrace x^a_1, \ldots, x^a_{k}\right\rbrace \cup \left\lbrace x^{a+1}_{1}, \ldots, x^{a+1}_k\right\rbrace$
    %         \item Define $\mathcal{B}^{-p}_r$ inductively as the sequence $\mathcal{B}^{-p-1}_r \setminus \left\lbrace b_a, b_{a+1} \right\rbrace \cup \left\lbrace b^*_a \right\rbrace$ for all $r$.
    %     \end{itemize}
    % \end{enumerate}
    % The result of this process is still $m$ total buckets, and all of the above techniques may be applied without a change to downsample resolution.

    % Consider $P$ a hyperparameter, and the sum of sum of square errors per bucket as the loss function. 

    % \begin{remark}
    %     Rather than serially splitting, and then combining buckets to arrive at the rebucketing, it's natural to ask how alternating these operations effects the result. The authors carried out several simulations of this technique and found that convergence to `stable' bucketing took place much more quickly, but produced far worse results with respect to total SSE.
    % \end{remark}


==> deprecated/graph_laplacians.tex <==
\section{Graph Laplacians}
%\textit{go over basics of graph laplacians}

Spectral graph theory is an integral facet of graph theory (\cite{chung1997spectral}) and one of the key objects of this theory is the Laplacian matrix of a graph, as well as its eigenvalues. 
% We review the basics of graph Laplacians and explain how we use their eigenvalues in this classification task. 
We assume all graphs are undirected and simple. For a graph $G$, let $A$ and $D$ be the adjacency matrix and the degree matrix of $G$ respectively.
% defined by
% \begin{equation*}
% A(u, v) = 
% \begin{cases}
% 1 & \text{if } u \text{ and } v \text{ are adjacent} \\
% 0 & \text{otherwise.}
% \end{cases}
% \end{equation*}
% Now define $D$ to be the diagonal matrix of degrees of vertices of $G$; i.e. $D(u, u) = d_u$, where $d_u$ is the degree of the vertex $u$. 
% \begin{equation*}
% L = D- A.
% \end{equation*}
The \emph{Laplacian} of $G$ is defined to be $L = D - A$. The \emph{normalized Laplacian} of $G$ is then defined to be $\tilde{L}  = D^{-1/2} A D^{-1/2}.$

Denote the eigenvalues(or \emph{spectrum}) of $\tilde{L}$ by  $0=\lambda_0 \leq \lambda_1 \leq \cdots \leq \lambda_{n-1}$. There is a well known connection between the spectrum of $\tilde{L}$ to properties of $G$:

\begin{theorem*}[Lemma 1.7, \cite{chung1997spectral}]\label{thm:graphspec}
For a graph $G$ with $n$ vertices, we have that
\begin{enumerate}
	\item $0 \leq \lambda_i \leq 2$, with $\lambda_0 = 0$. Further, $\lambda_{n-1} = 2$ if and only if  a connected component of $G$ is bipartite and nontrivial. 
	\item If $G$ is connected, then $\lambda_1 > 0$. If $\lambda_i = 0$ and $\lambda_{i+1} \neq 0$ then $G$ has exactly $i+1$ connected components.
\end{enumerate}
\end{theorem*}



%For an undirected, simple graph $G$, let $d_v$ denote the degree of the vertex $v$. The Laplacian of the graph $G$ is defined to be the matrix
%
%\begin{equation*}
%\tilde{L}(u, v) = 
%\begin{cases}
%d_v & \text{if } u = v \\
%-1 & \text{if } u \text{ and } v \text{ are adjacent} \\
%0 & \text{otherwise.}
%\end{cases}
%\end{equation*}


% The graph Laplacian can be used to engineer features of an input point cloud $X \subset \mathbb{R}^m$ for use in machine learning algorithms via constructing a multivariate sequence that captures topological structure, or relative connectedness with respect to distance, of the data over a varying range of resolutions.


\textbf{Persistent Laplacian Eigenvalues for Time Series Analysis}\label{sec:laplacians_ts} Denote by $\tilde{L}_{\epsilon}(X)$ the normalized Laplacian of $G_{\epsilon}(X)$. Define $\hat{\lambda}_{\epsilon}(X) = [ \lambda_{\epsilon}(X)_0, \lambda_{\epsilon}(X)_1, \dots \lambda_{\epsilon}(X)_{n-1} ]$ to be the vector of eigenvalues of $\tilde{L}_{\epsilon}(X)$, in ascending order: $0 = \lambda_{\epsilon}(X)_0 \leq \lambda_{\epsilon}(X)_1 \leq \cdots \leq \lambda_{\epsilon}(X)_{n-1} \leq 2$. When the context is understood, we will drop the designation $(X)$ in the above notations; e.g. $G_{\epsilon}$ or $\lambda_{\epsilon 0}$.

Let $I$ be an interval, $\hat{v} = [v_0, v_1, \dots, v_{n-1}]$ be a vector, and define 

\begin{equation}
\textbf{count}_{I}(v) : = \#\{ v_i \mid v_i \in I  \}.
\end{equation}
For a given interval $[0, r]$ (this will be our range of resolutions), and a finite collection of real numbers $0 = \tau_0 < \tau_1 < \cdots < \tau_k = 2$, define for $\epsilon \in [0, r]$:
\begin{equation}
\mu_j(\epsilon) := 
\begin{cases}
	\textbf{count}_{[\tau_j, \tau_{j + 1})}(\hat{\lambda_{\epsilon}}) \text{  for } 0 \leq j < k - 1 \\
	\textbf{count}_{[\tau_j, \tau_{j + 1}]}(\hat{\lambda_{\epsilon}}) \text{  for } j = k - 1.
\end{cases}
\end{equation}

\noindent That is, $\mu_j(\epsilon)$ counts the number of eigenvalues of $\tilde{L}_{\epsilon}$ that lie between $\tau_j$ and $\tau_{j + 1}$. Observe that $\textbf{count}_{[0, 0]}(\hat{\lambda_{\epsilon}})$ is equal to the number of connected components of $G_{\epsilon}$. We will view the collection $\{ \mu_j \}$ as a collection  of $j$ real-valued functions with domain $[0, r]$. Mirroring Sec. \ref{sec:ph_ts}, we refer to the collection of $\mu_j$'s as \emph{persistent Laplacian eigenvalues}. Given a time series $\{ f(t_i)  \}_{i=0}^n$ we form $T^m$, and compute $\{ \mu_j \}_{j=0}^l$ for some choice of $\tau_0, \dots \tau_l$.

==> deprecated/intro.tex <==
Topological Data Analysis (TDA) (\cite{computingPH},\cite{topo_persis}) has gained much attention due to applications for data analysis and machine learning. In particular, persistent homology (\cite{Scopigno04persistencebarcodes},\cite{Edelsbrunner2000TopologicalPA}) has been leveraged for machine learning purposes in numerous tasks. The methods attempt to describe the shape of the data in a latent space particularly amenable to feature engineering. The efficacy of topological features has been demonstrated in various tasks (\cite{Chazal2017AnIT}). 

In this paper, we investigate the performance of various topological feature engineering approaches for EEG time-series classification using one dimensional CNN as the classifiers. While CNN architectures are heavily experimented on, less research has explored models for feature engineering using modern geometric techniques (\cite{gcrn, geom_dl}). Usually, CNNs are trained on the raw time-series data where a convolutional kernels of a fixed sizes and strides are applied to the series with moving windows to compute higher-order features. Persistent homology of the {\em Takens' embedding} provides one geometric procedure to engineer features for a time-series (\cite{Umeda2017}). 

For a time-series, the $k$-dimensional {\em Takens' embedding} of the time-series is the Euclidean embedding of points defined by a sliding window of size $k$---this provides a point-cloud representation of the time-series. From this point cloud the usual TDA approach provides persistent features. Both the raw series and the persistent features can be exploited for machine learning tasks. As a first step towards better understanding feature engineering on time-series, we compare the performance of these two approaches for the classification task.

Furthermore, we propose a novel geometric method beyond homology theories utilizing eigenvalues of sequences of graph Laplacians. Again, we utilize the point-cloud representation's $\epsilon$-neighbor graph, and compute the normalized graph Laplacians' eigenvalues. Density counts of these eigenvalues are encoded as $m$ discrete $\epsilon$-series. We demonstrate the superiority of our approach over the homological features and compare to the raw time-series via classification experiments while keeping the classifier architecture fixed.   
	
Generally, CNN architectures are optimized via network features like batch size, learning rate, kernels, pooling layers, and the like. Some papers have experimented with resizing to improve training time --- in (\cite{DAWNBench}) they introduced dynamic resizing with progressive resolution; (\cite{DBLP}) have investigated the CNN robustness under noise. We have not found in the literature examinations of explicit downsampling algorithms' effects. To this effect, we study the performance of the feature engineering methods across multiple regimes of time-series resolution, and effective resolutions, comparing degradation across the feature types and downsampling methods–––a practice common in the signal processing literature but less so in classification of time-series. Note that the encoding methods in this paper need not only apply to sequential collections.

	The principle contributions of this work include:
	\begin{itemize}
		\item Introduce a new feature engineering technique utilizing latent geometric properties of the time series.
		\item Apply the theory and methods of downsampling to time-series classification problem. 
		\item Propose and demonstrate a comparison framework and baseline results for time series clustering via varying features and CNN architectures. 
	\end{itemize}
	
	\subsection{Comments and Caveats}

	In machine learning tasks, especially those with more complicated models, it is essential to attempt to establish a baseline, a set of target metrics, and a comparison pipeline for apples-to-apples evaluation\textemdash in some literature this is called boat-racing, or horse-racing. During our literature review of TDA methods for the EEG prediction dataset, we did not find sufficient comparators and thus integrate this into our experimentation goals, whence the large volume of experiments considered in this paper.

	We do not treat the neuroscience topics necessary for a deeper investigation of EEG technology or seizures. We treat the dataset as a mathematical task, and focus instead on the models and methods in machine learning. In particular, as highlighted in (\cite{GCN-EEG}) EEG datasets are structural time series, i.e. physical geometry of data collection correlates with relationships between series. We use only local readings to reduce this covariant structure. Furthermore, train and test splitting can be challenging as several samples are taken from the same patient. For these, and other reasons, we make no comparison to SOTA networks. 

	\subsection{This work in context}

	Generally, CNN architectures are optimized via network features like batch size, learning rate, kernels, pooling layers, and the like. Some papers have experimented with resizing to improve training time --- in (\cite{DAWNBench}) they introduced dynamic resizing with progressive resolution. Others (\cite{DBLP}) have investigated the robustness of CNN performance under image degradation due to noise, but we've not found in the literature examinations of explicit downsampling algorithms' effects.

	For a collection classification task, the encoding of the data itself is also at opportunity for tuning. While common approaches to sequential data sets use RNNs and LSTMs to take advantage of data characteristics like autoregressive features, the encoding methods in this paper need not only apply to sequential collections. 

	We wish to highlight that while time series classification is well studied and has clear and effective baselines (\cite{TSclass}), EEG classifiers are of great value and remain elusive. 
	
    \subsection*{Overview of model pipelines}
	
\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
    \includegraphics[width=.48\textwidth]{paper_materials/figures/raw_time_series_example.png}
    \caption{Raw time series from a segment of time where the patient's eyes were closed, segmented to 600 time steps, not downsampled.}
    \label{fig:raw_time_series}
    
    \includegraphics[width=.48\textwidth]{paper_materials/figures/eeg_eye_betti_numbers_example.png}
    \caption{$\beta_j(\epsilon)$ computed for the time series in Fig. \ref{fig:raw_time_series} as described in Section \ref{sec:ph_ts}.}
    \label{fig:pers_betti_nums}
    
    \includegraphics[width=.48\textwidth]{paper_materials/figures/eeg_eye_persistent_laplacian_example_area.png}
    \caption{Area plot of $\mu_j(\epsilon)$ for the time series in Fig. \ref{fig:raw_time_series} as described in Section \ref{sec:laplacians_ts}.}
  \label{fig:pers_lpn_eigs}
\end{wrapfigure}

% We outline the various feature pipelines to be fed into our CNN architectures:

	\textbf{Raw Time Series Features:} We feed the sequential series values into two kernel layers of one-dimensional convolution and max pool layers followed by a fully connected layer.

	\textbf{Persistent Betti Numbers Features:}	We encode each time series with the `k-step` Takens' embedding into $\mathbb{R}^k$. This point cloud's $\epsilon$-neighbor graph generates the Vietoris-Rips filtration up to dimension 3. The order of the degree $n$ simplicial homology (or $n$'th Betti number) is computed for each $\epsilon$ neighbor complex, and encoded as $n$ discrete $\epsilon$-series. We feed the sequential $\epsilon$-series values --- each on their own channel --- into two kernel layers of one-dimensional convolution and max pool layers followed by a fully connected layer.

	\textbf{Persistent Laplacian Eigenvalue Features:}	We encode each time series with the `k-step` Takens' embedding into $\mathbb{R}^k$. This point cloud's $\epsilon$-neighbor graph is collected and it's normalized graph Laplacians are computed. The eigenvalues of these Laplacians are computed and bucketed into a partition of $m$ buckets. The counts of eigenvalues in each bucket are encoded as $m$ discrete $\epsilon$-series. We feed the sequential $\epsilon$-series values --- each on their own channel --- into two kernel layers of one-dimensional convolution and max pool layers followed by a fully connected layer.

	\textbf{Downsampled input data:} In each of the pipelines, we prepend the model pipeline with a downsampling step using one of three downsampling algorithms and several downsampling resolutions. 

	\textbf{Experimental design:} Our design matrix consists of the three downsampling methods applied to $\left\lbrace 200, 300, 400, 500, 600\right\rbrace$ initial data resolutions downsampled by steps of $50$. Each of these initial data sets are fed through each of the model pipelines and subsequent CNNs. We use cross-validation and accuracy to evaluate the performance.

==> deprecated/introduction.tex <==
\section*{Introduction}
	Topological Data Analysis (TDA) (\cite{computingPH}, \cite{Scopigno04persistencebarcodes}, \cite{Edelsbrunner2000TopologicalPA}, \cite{topo_persis}) has emerged from Algebraic Topology as an approach to the problem of describing the shape of data. In recent years, TDA has gained much attention due to applications for data analysis and machine learning. In particular, persistent homology (\cite{topo_persis},\cite{Edelsbrunner2000TopologicalPA}) --- frequently in the form of barcodes --- has been leveraged for machine learning purposes in numerous tasks (\cite{Chazal2017AnIT}). Classification tasks seeking to label data collections so too frequently utilize the notion of the shape of data (in a latent geometry), via feature engineering. 

	In this paper, we investigate the performance of a one dimensional CNN on a binary classifying task for EEG data, under a collection of feature engineering approaches. While CNN architectures are heavily experimented on, less research has explored models for feature engineering using modern geometric techniques (\cite{gcrn, geom_dl}). We engineer and train networks using three types of features from the time series, investigating robustness of the classifiers to varying resolution and downsampling. We establish performance results across multiple regimes of EEG resolution, and effective resolutions, comparing degradation across the feature types. We also compare across differing downsampling methods: a practice common in the signal processing literature but less so in classification of time-series.

	Persistent homology of the Takens' embedding (c.f. \ref{sec:takens}) comprises the first set of engineered features (\cite{Umeda2017}). Unfortunately, the introduction of that approach lacked a comparison to current state of the art techniques, or even to standard techniques in the appropriately related tasks --- we fill that gap amidst our experiments. Our second feature set is a novel geometric method beyond that of traditional TDA methods utilizing eigenvalues of a sequence of graph Laplacians (c.f. \ref{sec:laplacians_ts}). We benchmark the performance of these two methods against a more modern method for time-series classification: a one dimensional CNN model trained on the time series data itself. We hold the classification network architecture constant to more directly evaluate the effectiveness of these features as estimators. 

	The principle contributions of this work include:
	\begin{itemize}
		\item Introduce a new feature engineering technique utilizing latent geometric properties of the time series
		\item Apply the theory and methods of downsampling to a time-series classification pipelines
		\item Propose and demonstrate a comparison framework and baseline results for time series clustering via varying features and CNN architectures
	\end{itemize}

	\subsection{Comments}

% 	In machine learning tasks, especially those with more complicated models, it is essential to attempt to establish a baseline, a set of target metrics, and a comparison pipeline for apples-to-apples evaluation\textemdash in some literature this is called boat-racing, or horse-racing. During our literature review of TDA methods for the EEG prediction dataset, we did not find sufficient comparators and thus integrate this into our experimentation goals, whence the large volume of experiments considered in this paper.

	We do not treat the neuroscience topics necessary for a deeper investigation of EEG technology or seizures. We treat the dataset as a mathematical task, and focus instead on the models and methods in machine learning. In particular, as highlighted in (\cite{GCN-EEG}) EEG datasets are structural time series, i.e. physical geometry of data collection correlates with relationships between series. We use only local readings to reduce this covariant structure. Furthermore, train and test splitting can be challenging as several samples are taken from the same patient. For these, and other reasons, we make no comparison to SOTA networks. 

	\subsection{This work in context}

	Generally, CNN architectures are optimized via network features like batch size, learning rate, kernels, pooling layers, and the like. Some papers have experimented with resizing to improve training time --- in (\cite{DAWNBench}) they introduced dynamic resizing with progressive resolution. Others (\cite{DBLP}) have investigated the robustness of CNN performance under image degradation due to noise, but we've not found in the literature examinations of explicit downsampling algorithms' effects.

	For a collection classification task, the encoding of the data itself is also at opportunity for tuning. While common approaches to sequential data sets use RNNs and LSTMs to take advantage of data characteristics like autoregressive features, the encoding methods in this paper need not only apply to sequential collections. 

	We wish to highlight that while time series classification is well studied and has clear and effective baselines (\cite{TSclass}), EEG classifiers are of great value and remain elusive. 

	\subsection{Overview of model pipelines}

% 	\begin{figure}[ht]
% 		\includegraphics[width=0.9\textwidth]{figures/V2cartoon.png}
%   		\caption{Three model pipelines; steps numbered as in telephone keypad; steps (2,3): raw time series CNN; steps (2,1,4,5,6): persistent Laplacian eigenvalues; steps (2,1,4,7,8,9): persistent Betti numbers.}
% 	   \label{fig:model_pipelines}
% 	\end{figure}
	
    \begin{figure}[ht]
    \centering
    
    \begin{minipage}{.5\textwidth}
      \centering
        \includegraphics[width=.95\textwidth]{paper_materials/figures/raw_time_series_example.png}
        \caption{Raw time series from a segment of time where the patient's eyes were closed, segmented to 600 time steps, not downsampled.}
        \label{fig:raw_time_series}
        
        \includegraphics[width=.95\textwidth]{paper_materials/figures/eeg_eye_betti_numbers_example.png}
        \caption{$\beta_j(\epsilon)$ computed for the time series in Fig. \ref{fig:raw_time_series} as described in Section \ref{sec:ph_ts}.}
        \label{fig:pers_betti_nums}
        
        \includegraphics[width=.95\textwidth]{paper_materials/figures/eeg_eye_persistent_laplacian_example_area.png}
        \caption{Area plot of $\mu_j(\epsilon)$ for the time series in Fig. \ref{fig:raw_time_series} as described in Section \ref{sec:laplacians_ts}.}
      \label{fig:pers_lpn_eigs}
    \end{minipage}%
    \begin{minipage}{.5\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{paper_materials/figures/TallCartoonwEx.png}
  		% \caption{Model pipelines}
	   \label{fig:model_pipelines}
    \end{minipage}
    \centering\captionsetup{justification=RaggedLeft}
    \caption{Model pipelines; steps (1,2): raw time series CNN; steps (1,3,4,5,6): persistent Laplacian eigenvalues; steps (1,3,4,7,8,9): persistent Betti numbers; Ex: $\epsilon$-neighbors graph construction}
    \end{figure}

	\textbf{Raw Time Series Features:} We feed the sequential series values into two kernel layers of one-dimensional convolution and max pool layers followed by a fully connected layer.

	\textbf{Persistent Betti Numbers Features:}	We encode each time series with the `k-step` Takens' embedding into $\mathbb{R}^k$. This point cloud's $\epsilon$-neighbor graph (c.f. Figure \ref{fig:model_pipelines} \textbf{Ex.}) generates the Vietoris-Rips filtration up to dimension 3. The order of the degree $n$ simplicial homology (or $n$'th Betti number) is computed for each $\epsilon$ neighbor complex, and encoded as $n$ discrete $\epsilon$-series. We feed the sequential $\epsilon$-series values --- each on their own channel --- into two kernel layers of one-dimensional convolution and max pool layers followed by a fully connected layer.

	\textbf{Persistent Laplacian Eigenvalue Features:}	We encode each time series with the `k-step` Takens' embedding into $\mathbb{R}^k$. This point cloud's $\epsilon$-neighbor graph is collected and it's normalized graph Laplacians are computed. The eigenvalues of these Laplacians are computed and bucketed into a partition of $m$ buckets. The counts of eigenvalues in each bucket are encoded as $m$ discrete $\epsilon$-series. We feed the sequential $\epsilon$-series values --- each on their own channel --- into two kernel layers of one-dimensional convolution and max pool layers followed by a fully connected layer.

	\textbf{Downsampled input data:}	In each of the pipelines, we prepend the model pipeline with a downsampling step using one of three downsampling algorithms and several downsampling resolutions. 

	\textbf{Experimental design:} Our design matrix consists of the three downsampling methods applied to $\left\lbrace 200, 300, 400, 500, 600,\right\rbrace$ initial data resolutions downsampled by steps of $50$. Each of these initial data sets are fed through each of the model pipelines and subsequent CNNs. We use cross-validation and accuracy to evaluate the performance.

%The current work seeks a few primary goals:
%\begin{enumerate}
%	\item Introduce "persistent eigenvalues" as a novel feature engineering method a la TDA.
%	\item Establish a baseline architecture for evaluation of these methods.
%	\item Analyze the sensitivity of the above with respect to data resolution.
%\end{enumerate}

==> deprecated/methods.tex <==
\section{Methods}
%\textit{go over basics of graph laplacians}

\subsection{Our Approach}
Spectral graph theory is an integral facet of graph theory (\cite{chung1997spectral}) and one of the key objects of this theory is the Laplacian matrix of a graph, as well as its eigenvalues. 
% We review the basics of graph Laplacians and explain how we use their eigenvalues in this classification task. 
We assume all graphs are undirected and simple. For a graph $G$, let $A$ and $D$ be the adjacency matrix and the degree matrix of $G$ respectively.
% defined by
% \begin{equation*}
% A(u, v) = 
% \begin{cases}
% 1 & \text{if } u \text{ and } v \text{ are adjacent} \\
% 0 & \text{otherwise.}
% \end{cases}
% \end{equation*}
% Now define $D$ to be the diagonal matrix of degrees of vertices of $G$; i.e. $D(u, u) = d_u$, where $d_u$ is the degree of the vertex $u$. 
% \begin{equation*}
% L = D- A.
% \end{equation*}
The \emph{Laplacian} of $G$ is defined to be $L = D - A$. The \emph{normalized Laplacian} of $G$ is then defined to be $\tilde{L}  = D^{-1/2} A D^{-1/2}.$

Denote the eigenvalues(or \emph{spectrum}) of $\tilde{L}$ by  $0=\lambda_0 \leq \lambda_1 \leq \cdots \leq \lambda_{n-1}$. Recall:

\begin{theorem*}[Lemma 1.7, \cite{chung1997spectral}]\label{thm:graphspec}
For a graph $G$ with $n$ vertices, we have that
\begin{enumerate}
	\item $0 \leq \lambda_i \leq 2$, with $\lambda_0 = 0$. Further, $\lambda_{n-1} = 2$ if and only if  a connected component of $G$ is bipartite and nontrivial. 
	\item If $G$ is connected, then $\lambda_1 > 0$. If $\lambda_i = 0$ and $\lambda_{i+1} \neq 0$ then $G$ has exactly $i+1$ connected components.
\end{enumerate}
\end{theorem*}



%For an undirected, simple graph $G$, let $d_v$ denote the degree of the vertex $v$. The Laplacian of the graph $G$ is defined to be the matrix
%
%\begin{equation*}
%\tilde{L}(u, v) = 
%\begin{cases}
%d_v & \text{if } u = v \\
%-1 & \text{if } u \text{ and } v \text{ are adjacent} \\
%0 & \text{otherwise.}
%\end{cases}
%\end{equation*}


% The graph Laplacian can be used to engineer features of an input point cloud $X \subset \mathbb{R}^m$ for use in machine learning algorithms via constructing a multivariate sequence that captures topological structure, or relative connectedness with respect to distance, of the data over a varying range of resolutions.


\textbf{Persistent Laplacian Eigenvalues for Time Series Analysis}\label{sec:laplacians_ts} Denote by $\tilde{L}_{\epsilon}(X)$ the normalized Laplacian of $G_{\epsilon}(X)$. Define $\hat{\lambda}_{\epsilon}(X) = [ \lambda_{\epsilon}(X)_0, \lambda_{\epsilon}(X)_1, \dots \lambda_{\epsilon}(X)_{n-1} ]$ to be the vector of eigenvalues of $\tilde{L}_{\epsilon}(X)$, in ascending order: $0 = \lambda_{\epsilon}(X)_0 \leq \lambda_{\epsilon}(X)_1 \leq \cdots \leq \lambda_{\epsilon}(X)_{n-1} \leq 2$. When the context is understood, we will drop the designation $(X)$ in the above notations; e.g. $G_{\epsilon}$ or $\lambda_{\epsilon 0}$.

Let $I$ be an interval, $\hat{v} = [v_0, v_1, \dots, v_{n-1}]$ be a vector, and define 

\begin{equation}
\textbf{count}_{I}(v) : = \#\{ v_i \mid v_i \in I  \}.
\end{equation}
For a given interval $[0, r]$ (this will be our range of resolutions), and a finite collection of real numbers $0 = \tau_0 < \tau_1 < \cdots < \tau_k = 2$, define for $\epsilon \in [0, r]$:
\begin{equation}
\mu_j(\epsilon) := 
\begin{cases}
	\textbf{count}_{[\tau_j, \tau_{j + 1})}(\hat{\lambda_{\epsilon}}) \text{  for } 0 \leq j < k - 1 \\
	\textbf{count}_{[\tau_j, \tau_{j + 1}]}(\hat{\lambda_{\epsilon}}) \text{  for } j = k - 1.
\end{cases}
\end{equation}

\noindent That is, $\mu_j(\epsilon)$ counts the number of eigenvalues of $\tilde{L}_{\epsilon}$ that lie between $\tau_j$ and $\tau_{j + 1}$. Observe that $\textbf{count}_{[0, 0]}(\hat{\lambda_{\epsilon}})$ is equal to the number of connected components of $G_{\epsilon}$. We will view the collection $\{ \mu_j \}$ as a collection  of $j$ real-valued functions with domain $[0, r]$. We refer to the collection of $\mu_j$'s as \emph{persistent Laplacian eigenvalues}. Given a time series $\{ f(t_i)  \}_{i=0}^n$ we form $T^m$, and compute $\{ \mu_j \}_{j=0}^l$ for some choice of $\tau_0, \dots \tau_l$.

% \subsubsection{Topological downsampling}

%     Given an \emph{n-step time-delay embeddings} of $\prescript{y}{}{x^j_i}$'s for those points in $b_j$, 

% \subsubsection{Dynamic Bucketing}


%     In the above bucketing strategies, points in all regions of the time series are given equal weight in the downsample. Often times, the lagging-variance of a time series is not uniform across the time-domain. One might expect that regions of higher variance might warrant higher resolutions in the downsample, while low variance might require lower resolutions. A simple implementation of this idea, \textit{(inspired by \cite{sveinn})} is demonstrated in Algorithm \ref{alg:dynamic bucketing}(implementation in Appendix). Downsampling methods are then applied to this bucketing of the timeseries.
    
%     \begin{algorithm}
%   \caption{Variance weighted dynamic bucketing
%     \label{alg:dynamic bucketing}}
%   \begin{algorithmic}[1]
%     \Require{$\mathcal{B}$ a naive bucketing, and $P$ an iteration count}
%     \Statex
%     \Function{dynamicbuckets}{$B:List[List[Float]$}
%       \Let{$[b_j]$}{$\mathcal{B}$} \Comment{$\left\lbrace x^j_i\right\rbrace_{1\leq i \leq k}=b_j$: buckets of $\mathcal{B}$}
%       \For{$i \gets 1 \textrm{ to } P$}
%         \For{$j \gets 1 \textrm{ to } m$}
%             \Let{$S(b_j)$}{$SSE(OLS(b_j))$}
%         \EndFor
%         \Let{$z$}{$\argmax_j(S(b_j))$}
%         \Let{$b^l_z$}{$\left\lbrace x^z_1, \ldots, x^z_{\floor{k/2}}\right\rbrace$}
%         \Let{$b^r_z$}{$\left\lbrace x^z_{\floor{k/2}+1}, \ldots, x^z_k\right\rbrace$}
%         \Let{$\mathcal{B}$}{$\mathcal{B}\setminus \left\lbrace b_z\right\rbrace \cup \left\lbrace b^l_z, b^r_z \right\rbrace$}
%       \EndFor
%       \For{$i \gets 1 \textrm{ to } P$}
%         \For{$j \gets 1 \textrm{ to } m+P$}
%             \Let{$S(b_j)$}{$SSE(OLS(b_j))$}
%         \EndFor
%         \Let{$a$}{$\argmin_a(S(b_a)+S(b_{a+1}))$}
%         \Let{$b^*_a$}{$\left\lbrace x^a_1, \ldots, x^a_{k}\right\rbrace \cup \left\lbrace x^{a+1}_{1}, \ldots, x^{a+1}_k\right\rbrace$}
%         \Let{$\mathcal{B}$}{$\mathcal{B}\setminus \left\lbrace b_a, b_{a+1} \right\rbrace \cup \left\lbrace b^*_a \right\rbrace$}
%       \EndFor
%       \State \Return{$\mathcal{B}$}
%     \EndFunction
%   \end{algorithmic}
% \end{algorithm}
    
    % \begin{enumerate}
    %     \item Consider again, the buckets of points ${b_j}$ as before, but call this sequence $\mathcal{B}_0$ \begin{itemize}
    %         \item Given points $\left\lbrace x^j_i\right\rbrace_{1\leq i \leq k}$ contained in the bucket $b_j$, compute the linear regression minimizing the sum of squares of the residuals to the model. Record this `loss' as $S(b_j)$.
    %         \item For $z=\argmax_j(S(b_j))$, denote $b^l_z=\left\lbrace x^z_1, \ldots, x^z_{\floor{k/2}}\right\rbrace$, and $b^r_z=\left\lbrace x^z_{\floor{k/2}+1}, \ldots, x^z_k\right\rbrace$
    %         \item Define $\mathcal{B}_p$ inductively as the sequence $\mathcal{B}_{p-1}\setminus \left\lbrace b_z\right\rbrace \cup \left\lbrace b^l_z, b^r_z \right\rbrace$
    %     \end{itemize}
    %     \item Assume now buckets $b_j$ from $\mathcal{B}_p$ but we purposely do not take care to notate different values of $k$ depending on $j$. \begin{itemize}
    %         \item Given points $\left\lbrace x^j_i\right\rbrace_{1\leq i \leq k}$ contained in the bucket $b_j$, compute the linear regression minimizing the sum of squares of the residuals to the model. Record this `loss' as $S(b_j)$.
    %         \item For $a=\argmin_a(S(b_a)+S(b_{a+1}))$, denote $b^*_a = \left\lbrace x^a_1, \ldots, x^a_{k}\right\rbrace \cup \left\lbrace x^{a+1}_{1}, \ldots, x^{a+1}_k\right\rbrace$
    %         \item Define $\mathcal{B}^{-p}_r$ inductively as the sequence $\mathcal{B}^{-p-1}_r \setminus \left\lbrace b_a, b_{a+1} \right\rbrace \cup \left\lbrace b^*_a \right\rbrace$ for all $r$.
    %     \end{itemize}
    % \end{enumerate}
    % The result of this process is still $m$ total buckets, and all of the above techniques may be applied without a change to downsample resolution.

    % Consider $P$ a hyperparameter, and the sum of sum of square errors per bucket as the loss function. 

    % \begin{remark}
    %     Rather than serially splitting, and then combining buckets to arrive at the rebucketing, it's natural to ask how alternating these operations effects the result. The authors carried out several simulations of this technique and found that convergence to `stable' bucketing took place much more quickly, but produced far worse results with respect to total SSE.
    % \end{remark}


==> deprecated/past_work.tex <==
\section{Past Work}
In (\cite{Umeda2017}), the author calculates persistent Betti numbers of EEG time series signals via the aforementioned Persistent Betti-number model pipeline before feeding the output into a CNN for an eyes open/closed prediction task. In particular, for time series $\{ f(t_i)  \}_{i=0}^n$, consider $T^m$ its Takens' embedding as the enumerated subset in $\mathbb{R}^m$, then compute $\beta_{k}(\epsilon)$ for all $0 \leq k < m$ and $\epsilon \in [0,r]$.

==> deprecated/persistent_homology.tex <==
\section{TDA for machine learning}


\subsection{Persistent Homology}
\label{ph}

% Fix $\epsilon \geq 0$, and let $X = \{ x_1, \ldots, x_n \}$ be an enumerated subset of $\mathbb{R}^m$. For $k = 0, 1, \ldots$ define $C_{\epsilon, k}$ to be the $\mathbb{R}$-vector space whose formal basis is given by all subsets of $X$ of the form 
% \begin{equation*}
% \{ (x_{i_0}, x_{i_1}, \ldots, x_{i_k}) \text{ such that } i_0 < i_1 < \cdots < i_k \text{ and } \norm{x_{i_{\alpha}} - x_{i_{\beta}}}  < \epsilon \text{ for all } \alpha, \beta = 0, 1, \ldots, k \}.
% \end{equation*}
% We take $C_{\epsilon, k}$ to be the zero vector space if there are no such subsets. There are linear maps $\partial_{k}: C_{\epsilon, k} \rightarrow C_{\epsilon, k-1}$ defined by

% \begin{equation*}
%     \partial_{\epsilon, k}(x_{i_0}, \dots, x_{i_k}) = \sum_{j = 0}^{k}(-1)^j(x_{i_0}, \ldots, \widehat{x_{i_j}}, \ldots, x_{i_k})
% \end{equation*}

% \noindent where $(x_{i_0}, \ldots, \widehat{x_{i_j}}, \ldots, x_{i_k})$ denotes the element $( x_{i_0},\ldots, x_{i_{j-1}}, x_{i_{j+1}},\dots, x_{i_k} ) \in C_{\epsilon, k-1}$. One can check that $\text{Im}(\partial_{\epsilon, k+1}) \subseteq \text{Ker}(\partial_{\epsilon, k})$. The \emph{$k^{th}\: \epsilon$-homology group} of $X$ is defined to be the vector space quotient $\text{H}_{\epsilon, k}(X) := \text{Ker}(\partial_{\epsilon, k})/\text{Im}(\partial_{\epsilon, k+1})$. The \emph{$k^{th}\: \epsilon$-Betti number} of $X$ is defined to be $\beta_{\epsilon, k}(X) := \text{dim}(\text{H}_{\epsilon, k}(X))$. Intuitively, $\beta_{\epsilon, k}(X)$ measures the number of $k$-dimensional holes in the point cloud $X$ at resolution $\epsilon$. We will typically write $\beta_k(\epsilon)$, and allow $\epsilon$ to vary over a fixed range $[0, r]$. We will also refer to $\beta_k(\epsilon)$ as an $\epsilon$-series. In the sequel, \emph{persistent homology} will in general refer to the collection of $\beta_k$'s, as they capture information about how the homology persists over varying resolutions. (c.f. \cite{Hatcher})


% Given a collection of data points in some $n$-dimensional space-often referred to as a point cloud-one might expect that they lie on some particular submanifold, and that the geometric structure of that submanifold contains important information about that data. 

% From a point cloud in a semimetric space with distance $\norm{-}$, frequently euclidean, construct a neighbors graph with respect to a parameter $\epsilon \in \mathbb{R}^{\geq 0}$, consisting of edges between any two data points separated by less than $\epsilon$. This graph is a 1-simplex in the language of topology, i.e. a set of points and edges such that all edges' boundaries are also contained in the set. We then consider all triples of points which are pairwise connected-cycles-and add the 2-dimensional faces with the edges as the boundaries. This procedure produces a 2-simplex. Similarly, we iteratively construct the higher simplices; lines, triangles, etc. More succinctly: consider $n$ faces of dimension $(n-1)$ which are co-incident on $(n-2)$-dimensional faces, and add the $n$-dimensional face with them as its boundary; this is the Rips complex (c.f. Figure  \ref{fig:model_pipelines} \textbf{Step 7.}). 

% Given a complex as above, consider the degree of the simplicial homology --- referred to as the Betti numbers. For all dimensions, these Betti numbers represent geometric invariants of the underlying complex, and thus the submanifold the points lie on. Thus, the complex, and the original neighbors graph, generates a sequence of nonnegative integers.

% Recall that we fixed the parameter $\epsilon$. As we change $\epsilon$, we change this sequence of numbers. The collection of Betti numbers as we range over $\epsilon$ is referred to as a \textit{barcode} of the persistent homology.

	
	
\textbf{Takens' Embedding}\label{sec:takens} Given a time series, $\{t_i \}_{i=0}^n \subset \mathbb{R}$, and a function $f: \mathbb{R} \rightarrow \mathbb{R}$. Then the \emph{Takens' embedding} with window size $m$, denoted $T^m$, is the collection of points in $\mathbb{R}^m$ given by
	\begin{equation*}
	\left\{  
		\left[ f(t_0), f(t_1), \dots, f(t_{m-1})  \right], 
		\left[ f(t_1), f(t_2), \dots, f(t_{m}) \right],  
		\dots,  
		\left[ f(t_{n-m+1}), f(t_{n - m +1}), \dots f(t_{n}) \right] 
	\right\} 
	\end{equation*}
\noindent That is, $T^m$ is the collection of points in $\mathbb{R}^m$ given by taking sliding windows over the time series $f(t_i)$. For volatile series, smooth transformations on this geometry are known to preserve properties of the time series, such as the dimension of chaotic attractor, and Lyapunov exponents of the dynamics.

\textbf{$\epsilon$-neighbor graph} Given a finite subset $X \subset \mathbb{R}^m$ with $n$ points, and a real number $\epsilon \geq 0$ we form the $\epsilon$-graph $G_{\epsilon}(X)$ with nodes of $G_{\epsilon}(X)$ indexed by the elements of $X$, and edges $v_x\rightarrow v_y$ for $x, y \in X$ if and only if $\norm{x - y} < \epsilon$.

% 	In the above, we began with a cloud of points; in contrast, the EEG data consists of a set of time series, which are each a 1-dimensional embedding, and thus lack much of the geometry we used to generate a complex. In the context of time series, it's common to consider their stochasticity; i.e. to what degree does a series' previous values predict the future values. Methods of auto-regression and de-trending are natural attempts to use these relationships for prediction. Perhaps the simplest strategy would be to consider series described by Markovian processes, i.e. that the next value is purely determined by the current value. In this simple model, one expects that all of the autoregression and trend may be modeled by the relationship of consecutive pairs of points. This leads naturally to a geometric encoding:
	
% 	Suppose we have a collection 



 
\textbf{Persistent Homology and Time Series Analysis}\label{sec:ph_ts} In (\cite{Umeda2017}), the author calculates persistent Betti numbers(c.f. the appendix: \ref{ph} for definitions) of EEG time series signals via the aforementioned Persistent Betti-number model pipeline before feeding the output into a CNN for an eyes open/closed prediction task. In particular, for time series $\{ f(t_i)  \}_{i=0}^n$, consider $T^m$ its Takens' embedding as the enumerated subset in $\mathbb{R}^m$, then compute $\beta_{k}(\epsilon)$ for all $0 \leq k < m$ and $\epsilon \in [0,r]$.

% 	Once these time-delay embeddings are constructed for all windows of points, they form a point cloud which may be fed through the machinery of persistent homology described above. This feature engineering thus converts a time series to a series of sequences of nonnegative integers. Note that the series of sequences is indexed by the $\epsilon$ values, and no longer the time steps of the original time series.

% 	While simple, we'll see that these geometric models capture enough information about the time series to produce impressive performance on classification tasks. One could easily imagine more sophisticated time series featurizations to generate the embeddings. We will examine a few with inspiration from state-space models in a forthcoming paper.

%\subsubsection{CNN Architecture}
%\label{betti_cnn}
%	The architecture for the CNN used in the setting of Betti numbers is as follows. First, a 1-dimensional multi-channel convolution layer, followed by a max pool layer, and ReLU layer. Next, a 1-dimensional multi-channel convolution layer, followed by a max pool layer, and ReLU layer. Finally a single fully connected layer with two nodes is used as the last layer. Cross-entropy loss is used when training the model.
%  

==> deprecated/results.tex <==
\section{Experiments}
% In this section we describe the experiments run using methods described in previous sections. We describe the data set used, as well as the neural net architectures used for three methods. We then describe the experiments involving classifying time series data across multiple downsampling resolutions, and give the results of these experiments.

\textbf{Data set and classification task} The data used in this work are time series EEG signals, and are provided by the University of Bonn, explored in \cite{eeg_data}. This data set is comprised of five sets (labeled A-E), each containing 100 single-channel EEG segments 23.6 seconds in duration, with 4097 observations. The segments were hand selected from within a continuous multi-channel EEG recording, chosen for absence of artifacts as well as fulfilling a stationarity condition. Set E contains segments of seizure activity, sets C and D are taken from epilepsy patients during an interval where no seizure activity was occurring, and sets A and B are observations from non epilepsy diagnosed patients. The observations in set A occur during times when the patient's eyes were open, while those in set B occur during times when the patient's eyes were closed. We study the classification task of A vs. B.

		
\textbf{CNN architectures} All of the prediction algorithms  used in this paper are CNNs, each with two sets of one dimensional convolution and max pool layers, followed by a fully connected layer to predict the class label. Architecture parameters are vectors representing $\left<\textrm{input},\textrm{channels},\textrm{factor},\textrm{kernel1 size},\textrm{kernel2 size}\right>$; $\left<\textrm{res},1,5,(\textrm{res}/600)*18,2\right>,\left<300,3,7,6,2\right>,\left<300,7,3,6,2\right>$ for raw time-series, Bettis, and eigenvalues respectively. \texttt{factor} refers to the multiplicative factor of input channels to output channels in each convolution layer, and \texttt{res} refers to the resolution to which the time series was downsampled to. Stride and dilation in both conv layers are 1 for each model; first pooling layer has size 7, second has size 3; each model is trained for 10 epochs.
		



% \begin{table}[H]
% \caption{CNN Architectures}
% \centering
% % \small
% \begin{tabular}{llll}
% \toprule
% features &      raw time series & persistent homology & persistent eigenvalues \\
% \midrule
% input size          &           res &                 300 &                    300 \\
% conv1 in channels   &                    1 &                   3 &                      7 \\
% conv channel factor &                    5 &                   7 &                      3 \\
% conv1 kernel size   &  (res/600)*18 &                   6 &                      6 \\
% conv2 kernel size   &                    2 &                   2 &                      2 \\
% \bottomrule
% \end{tabular}
% \label{table:cnn_architectures}
% \end{table}

%In this subsection we describe the neural net architecture used for the classification task (A vs. B) where the input to the neural net is the time series itself. The architecture used is a CNN with one dimensional convolutions. There are two convolution-max pool layers followed by 
%
%The architecture for the CNN used in the setting of the raw time series is as follows. First, a 1-dimensional single-channel convolution layer, followed by a max pool layer, and ReLU layer. Next, a 1-dimensional multi-channel convolution layer, followed by a max pool layer, and ReLU layer. Finally a single fully connected layer with two nodes is used as the last layer. Cross entropy loss is used when training the model.		

%            network_parameter_spec = NetworkParameterSpec(
%                input_size=parameter_spec.ds_resolution,
%                conv1_in_channels=1,
%                conv_channel_factor=5,
%                conv1_kernel_size=math.floor((parameter_spec.ds_resolution/600)*18.),
%                conv1_stride=1,
%                conv1_dilation=1,
%                conv2_kernel_size=2,
%                conv2_stride=1,
%                conv2_dilation=1,
%                pool_size1=7,
%                pool_size2=3,
%                num_epochs=10,
%                name='raw_time_series',
%                feature_labels=['A', 'B'],
%                target=['A'],
%            )
		
%\subsection{CNN for Persistent Homology Features}
%\label{betti_cnn}
%The architecture for the CNN used in the setting of Betti numbers is as follows. First, a 1-dimensional multi-channel convolution layer, followed by a max pool layer, and ReLU layer. Next, a 1-dimensional multi-channel convolution layer, followed by a max pool layer, and ReLU layer. Finally a single fully connected layer with two nodes is used as the last layer. Cross entropy loss is used when training the model.

%network_param_spec = NetworkParameterSpec(
%    conv1_in_channels=1,
%    conv_channel_factor=7,
%    conv1_kernel_size=6,
%    conv1_stride=1,
%    conv1_dilation=1,
%    conv2_kernel_size=2,
%    conv2_stride=1,
%    conv2_dilation=1,
%    pool_size1=7,
%    pool_size2=3,
%    fc_in_features_size=28714,
%    num_epochs=10,
%    name='umeda',
%    feature_labels=['A', 'B'],
%    target=['A'],
%)

%\subsection{CNN for Graph Laplacian Features}
%\label{laplacian_cnn}

%network_param_spec = NetworkParameterSpec(
%    input_size=300,
%    conv1_in_channels=7,
%    conv_channel_factor=3,
%    conv1_kernel_size=6,
%    conv1_stride=1,
%    conv1_dilation=1,
%    conv2_kernel_size=2,
%    conv2_stride=1,
%    conv2_dilation=1,
%    pool_size1=7,
%    pool_size2=3,
%#     fc_in_features_size=18018,
%    num_epochs=10,
%    name='lpn_eigvals',
%    feature_labels=['A', 'B'],
%    target=['A'],
%)

\textbf{Experiments and Results} For a given chunk size, downsampling method, and downsampling rate, we run 10-fold cross validation for each of the three prediction methods described. The average and standard deviation of accuracy is recorded and displayed in Figure \ref{fig:perf_non_dynamic} for non-dynamic bucketing downsampling methods, and Figure \ref{fig:perf_dynamic} for dynamic bucketing downsampling methods.

% \subsection{Results}
% We present here experimental results under various feature sets:

\begin{figure}[ht]
\centering
\includegraphics[width=0.75\textwidth]{paper_materials/figures/eeg_eye_results_non_dynamic_v2.png}
\caption{Experiment results for non dynamic bucketing downsampling methods.}
\label{fig:perf_non_dynamic}
\end{figure}

% With dynamic downsampling

% \begin{figure}[ht]
% \includegraphics[width=0.9\textwidth]{paper_materials/figures/eeg_eye_results_dynamic_v2.png}
% \caption{Experiment results for dynamic bucketing downsampling methods.}
% \label{fig:perf_dynamic}
% \end{figure}

% \begin{figure}[ht]
% \includegraphics[width=0.9\textwidth]{paper_materials/figures/raw_time_series_example.png}
% \caption{Raw time series.}
% \label{fig:perf_dynamic}
% \end{figure}

% \begin{figure}[ht]
% \includegraphics[width=0.9\textwidth]{paper_materials/figures/betti_numbers_example.png}
% \caption{Betti numbers.}
% \label{fig:perf_dynamic}
% \end{figure}

% \begin{figure}[ht]
% \includegraphics[width=0.9\textwidth]{paper_materials/figures/eigenvalues_bucketed_example.png}
% \caption{Persistent eigenvalues.}
% \label{fig:perf_dynamic}
% \end{figure}

%	\subsection{Sequence for seizure prediction}
%	\subsection{Sequence for eyes open/closed prediction}
